Exposure Bias versus Self-Recovery: Are Distortions Really Incremental for Autoregressive Text Generation?

Exposure bias has been regarded as a central problem for auto-regressive language models (LM). It claims that teacher forcing would cause the test-time generation to be incrementally distorted due to the training-generation discrepancy. Although a lot of algorithms have been proposed to avoid teacher forcing and therefore alleviate exposure bias, there is little work showing how serious the exposure bias problem actually is. In this work, we focus on the task of open-ended language generation, propose metrics to quantify the impact of exposure bias in the aspects of quality, diversity, and consistency. Our key intuition is that if we feed ground-truth data prefixes (instead of prefixes generated by the model itself) into the model and ask it to continue the generation, the performance should become much better because the training-generation discrepancy in the prefix is removed. Both automatic and human evaluations are conducted in our experiments. On the contrary to the popular belief in exposure bias, we find that the the distortion induced by the prefix discrepancy is limited, and does not seem to be incremental during the generation. Moreover, our analysis reveals an interesting self-recovery ability of the LM, which we hypothesize to be countering the harmful effects from exposure bias.

==> discuss.tex <==
\section{Limitations and Discussion}

What is reason that exposure bias becomes a well-known belief? ... talk about MLE objective ... $KL(P||Q)$ ... While it's true that training is ``exposed" to data history, the training not necessarily ``biased".

==> emnlp2021_response/response.tex <==
=== General ===

We sincerely thank all reviewers for their helpful comments! Please refer to our response to each individual reviewer.

=== R1 ===

Thanks for the review!

Re "What is the average length of samples? The wiki-103 dataset used in the experiment has long paragraphs, where some samples even contains more than 1000 words. However, in the experiments, the largest prefix length is 100..."

Well it depends on how you define "samples". In this work we treat each wiki paragraph as a sample, where the average length in the dataset is around 120. The average length of documents are around 3380. However, it will be difficult for us to fit sequences that long into memory. We think length 100 is fairly long by common sense.  Since errors from exposure bias do not build up in length 100, and considering the self-recovery ability shown in Section 6.4, we really do not see any strong reason to make the prefix even longer.

Re additional citations:

We will add the citations, thanks!


=== R2 ===

Thanks for the review!

Re " only attempted classical ancestral sampling ... In practical applications, beam search / top-k / top-p sampling are widely used. Will the same results hold for those?":

We have conducted experiments with top-k sampling for EB-M (line 451) and human evaluation (line 552), where the observations are consistent with ancestral sampling. We don't think beam-search is widely used for open-ended generation, because it would lead to serious repetitions [1]. Moreover, as shown in Figure 4 of [1], the repetition also happens with human generated text, i.e., it's not due to exposure bias. Due to these reasons, we did not test with beam-search.

Re "The experiment with a prefix being random or shuffled might not indicate the non-existence of exposure bias":

Yes, we did not say this disprove exposure bias. We only state that this self-recovery behavior is unexpected and casts doubt on the seriousness of EB. We completely agree that these inputs are extreme and we only design them for experiment purpose. In Section 6.4, we tested with softer versions of noises (e.g., corrupt rate 0.3), which we also observe the model could self-recover from.

Re "I'm worried that some outlier ratio values may dominate the final EB-M result. ... Have the authors tried BLEU-4, BLEU-3, BLEU-2, BLEU-1?":

(1) For EB-M ratios, we show the standard deviation from 10 runs with different random seeds (line 427) in Table 2. The std are all very small (< 0.01), and actually in all runs we get values very close 1, so there was no outlier value. (2) Yes, we have tested with BLEU-4/2/1, and the measurements are very similar to the BLEU-3 results reported. Also note that our observations are consistent with a number of various NLG metrics. We will add this to the paper.

Re "why Ross et al. (2011), the theoretically-proven classic imitation learning result that errors compound, doesn't hold in the text generation case":

We assume the reviewer is referring to theorem 2.1 of [https://www.ri.cmu.edu/pub_files/2011/4/Ross-AISTATS11-NoRegret.pdf]. Note that the this theorem is an upper bound for the errors, i.e., it does not guarantee that errors would compound. Also, this theorem clearly can not explain the self-recovery ability shown in our work. 

Re "discuss more on the impact of prefix length in the experiments?":

Exposure bias claims that distortions from model's generation should be incremental. Therefore, we vary the prefix length, and check whether the performance gap becomes larger. We stated this methodology in line 370-371.  

Re " Is it possible that the same phenomenon might not hold in other tasks? It will be great if the authors can qualify the scope":

Yes, we have stated this work is focused on open-ended language generation in the first line of abstract, and the beginning of Section 3 (background). We have also stressed this limitation in Section 7 (Limitations), where we explicitly write that "exposure bias could be more serious in other applications of different nature".

Re additional citations:

We will add the citations, thanks!

Re self-recovery:

Finally, we are concerned that in the review Section 6.4 is not mentioned. We regard it as an important and interesting part of our work because the existence of self-recovery echoes (or supports) the weak impact from EB. If you skipped it, we would really appreciate if you could check it out.

[1] THE CURIOUS CASE OF NEURAL TEXT DeGENERATION

==== R3 ===

Thanks for the review!

Re "For EB-C, synthetic data is generated by a Transformer, how about LSTM?":

Yes we also have EB-C results on LSTM. In Figure 4 (Appendix C), the synthetic data are from a LSTM (also the model is a LSTM). The observations for the MLE-trained model are similar to the transformer model.

Re "My only concern is for EB-C, the score is based on synthetic dataset that is generated by another language model. a little bit weird.":

As explained in section 5.2, having access to the data distribution helps us judge the quality of the model's conditional distribution given any prefix. Moreover, the synthetic EB-C results are consistent with observations from the human evaluation for consistency in Section 6.3.

Re "The length of prefix and prompts are fixed in experiments.":

We have varied the prefix length from 20 to 100. The prompt length are fixed to 20, because it shouldn't affect measurement of exposure bias (prompts are fed to both the data prefix or model prefix case).


==> emnlp2021_response/reviews.tex <==
============================================================================ 
EMNLP 2021 Reviews for Submission #1614
============================================================================ 

Title: Exposure Bias versus Self-Recovery: Are Distortions Really Incremental for Autoregressive Text Generation?
Authors: Tianxing He, Jingzhao Zhang, Zhiming Zhou and James Glass


============================================================================
                            REVIEWER #1
============================================================================

What is this paper about, what contributions does it make, and what are the main strengths and weaknesses?
---------------------------------------------------------------------------
This paper propose a method to measure how serious the exposure bias problem actually is. Specifically, they respectively use the data and model output as prefix and calculate the score of the generated suffix given the prefix. Comparing the scores of the generated suffix given different prefixes, the authors draw the conclusion that the exposure bias is not a big problem since the language model has a self-recovery ability. 

The paper is well written, and the conclusion is surprising and counterintuitive. As for the weakness, I have a concern about the experimental setting. The wiki-103 dataset used in the experiment has long and complex paragraphs from Wikipedia, where some samples even contains more than 1000 words. However, in the experiments, the largest prefix length is 100, which may only contain less than 10\% words of the sample. If this is true, then the prefix is too low to measure the exposure bias. As the sample length varies among samples, I suggest not setting a fixed prefix length, but use a prefix length with a fixed proportion of the sample. For example, you can report EB scores with the prefix length of 10%, 20%, 50%, ... of the sample length.
---------------------------------------------------------------------------


Reasons to accept
---------------------------------------------------------------------------
Well written paper with a surprising and counterintuitive conclusion.
---------------------------------------------------------------------------


Reasons to reject
---------------------------------------------------------------------------
1. The experiment setting is not very convincing.
2. As the authors admit, this work is only focused on open-ended language generation and the conclusion is not applicable to other NLG tasks.
---------------------------------------------------------------------------


Questions for the Author(s)
---------------------------------------------------------------------------
1. What is the average length of samples?
---------------------------------------------------------------------------


Missing References
---------------------------------------------------------------------------
These non-MLE works that support greedy search or sampling during training should also be discussed:
1.Trainable Greedy Decoding for Neural Machine Translation
2.Greedy Search with Probabilistic N-gram Matching for Neural Machine Translation
3.Differentiable Sampling with Flexible Reference Word Order for Neural Machine Translation
4.Guiding teacher forcing with seer forcing for neural machine translation
This paper use a similar approach to analyze the effect of prefix, but they do not study the exposure bias problem:
1.What Context Features Can Transformer Language Models Use?
---------------------------------------------------------------------------


---------------------------------------------------------------------------
Reviewer's Scores
---------------------------------------------------------------------------
                         Reproducibility: 4
     Overall Recommendation - Long Paper: 3.5


============================================================================
                            REVIEWER #2
============================================================================

What is this paper about, what contributions does it make, and what are the main strengths and weaknesses?
---------------------------------------------------------------------------
For neural autoregressive sequence models, at training time, MLE + teaching forcing is commonly used where the prefix is the data. However, at generation-time, the prefix is from the model. This â€œexposure biasâ€  mismatch is investigated. The term has always been defined casually in the text generation community. Prior works havenâ€™t rigorously studied this problem in the context of text generation. The author proposes quantitative measures for exposure bias Eq. (2) after which the authors discussed its limitations, and Eq. (4). Quantitative results and human evaluations found that using a model-generated prefix vs. a data prefix, the difference is minor.  


Strengths

- More serious discussion on the exposure bias problem would definitely benefit the text generation community. Researchers have used the term "exposure bias" casually for years. 

- The authors discuss the limitation of EB-M well, and discuss the limitations of their work well, which could be of great interest to the research community.

- The writing is clear.


Weaknesses and comments 

- The experiments are on open-ended text generation. Is it possible that the same phenomenon might not hold in machine translation /  summarization / question generation / etc.? It will be great if the authors can qualify the scope of the title/abstract. 

- The authors only attempted classical ancestral sampling without invoking sampling algorithms. However in most practical applications, beam search / top-k / top-p sampling are widely used. Will the same results hold using those decoding algorithms? The authors say that they donâ€™t use those sampling algorithms because the algorithms are known to â€œtrade quality out of diversity.â€  In many tasks people do not want diversity. Sometimes one correct generation is enough. Moreover, I donâ€™t believe itâ€™s proven that using those sampling algorithms will lead to smaller "exposure bias." For example sometimes when using non-ancestral-sampling, there will be repetitions and hallucinations. 

- On the qualitative attempt: the â€œprefix being random or shuffledâ€  might lead to better behavior than â€œprefix being model-generated.â€  The experiment corresponding to the â€œprefix being random or shuffledâ€  case might not indicate the non-existence of exposure bias. Itâ€™s possible that in the former case, the prefix is so messy (and almost never empirically take place in real applications) that perhaps the models just give up on using the prefix. In the latter case, the prefix is meaningful so the models may continue talking about an incorrect topic (i.e., already-deviated topic), for example.

- Minor: It might be helpful to include some of the important details (how long the prefix is, etc.) early in Section 4.  

- The intention for f-score is that the higher the score, the better the quality/diversity. Although in general, higher BLEU means higher quality. However, Iâ€™m worried that some outlier ratio values may dominate the final result. Whatâ€™s the histogram/distribution of the EB-M? Iâ€™m also a bit concerned at the quality of sentence-level BLEU. Have the authors tried BLEU-4, BLEU-3, BLEU-2, BLEU-1, for example, on the sentence-level, and compare whether the results are consistent? 

- A smaller CGD value indicates a better-modeled conditional distribution for W_{l+1} under p_H - this depends on what â€œbetter-modeledâ€  means? Comparing â€œ99% of words in the vocab have minimal difference with p_D & 1% of words are very wrongâ€  vs. â€œmany words have very different probability compared to p_Dâ€  perhaps the former will have a smaller divergence but the impact to the "quality" might be bigger. 

- A bit more discussion on why Ross et al. (2011), the theoretically-proven classic imitation learning result that errors compound, doesnâ€™t hold in the text generation case. 

- Not necessary in this article if the authors discuss the relevant limitations / qualify their abstract+introduction: testing on another dataset or even another task would be great.
---------------------------------------------------------------------------


Reasons to accept
---------------------------------------------------------------------------
More serious discussion on the exposure bias problem would definitely benefit the text generation community. Researchers have used the term "exposure bias" casually for years.
---------------------------------------------------------------------------


Reasons to reject
---------------------------------------------------------------------------
Please see "weaknesses."
---------------------------------------------------------------------------


Questions for the Author(s)
---------------------------------------------------------------------------
- Can the authors discuss more on the impact of prefix length in the experiments? 

- Do the authors have any intuition / brief comments on why Ross et al. (2011), the theoretically-proven classic imitation learning result that errors compound, doesnâ€™t hold in the text generation case?
---------------------------------------------------------------------------


Missing References
---------------------------------------------------------------------------
- Lin et al. (2020): https://aclanthology.org/2020.emnlp-main.494/

- (Can be considered contemporaneous work:) Pang and He (2021): https://openreview.net/pdf?id=RovX-uQ1Hua
---------------------------------------------------------------------------


---------------------------------------------------------------------------
Reviewer's Scores
---------------------------------------------------------------------------
                         Reproducibility: 3
     Overall Recommendation - Long Paper: 3


============================================================================
                            REVIEWER #3
============================================================================

What is this paper about, what contributions does it make, and what are the main strengths and weaknesses?
---------------------------------------------------------------------------
This paper studies the exposure bias for auto-regressive generation. Surprisingly, their automatic and human evaluations show that exposure bias is not as serious as we thought before. They further demonstrate that language models have the ability to recover when unreasonable prefix is given. It leads to the conclusion that exposure bias may exist, but can be recored by language model themselves, therefore it is not as serious as we expect.

The author study an interesting problem and propose a reasonable way to quantize the influence of exposure bias. My only concern is that for EB-C, they evaluate the score based on synthetic dataset that is generated by another language model. This is a little bit weird.
---------------------------------------------------------------------------


Reasons to accept
---------------------------------------------------------------------------
- The research question is interesting.
- They propose reasonable approach to quantize the influence of exposure bias.
- The results compared with shuffled data are convincing.
---------------------------------------------------------------------------


Reasons to reject
---------------------------------------------------------------------------
- The evaluation of EB-C requires synthetic data.
- The length of prefix and prompts are fixed in their experiments. It would be interesting if the author can provide more studies on this.
---------------------------------------------------------------------------


Questions for the Author(s)
---------------------------------------------------------------------------
- For EB-C, given that the synthetic data is generated by a Transformer, if we consider weaker language models, such as LSTM, does the exposure bias become more serious?
---------------------------------------------------------------------------


---------------------------------------------------------------------------
Reviewer's Scores
---------------------------------------------------------------------------
                         Reproducibility: 4
     Overall Recommendation - Long Paper: 3


==> sec_conditional-method.tex <==
\vspace{-0.25cm}
%\section{A Quantification Approach using Conditional Distribution}
\section{Word-level Quantification}
\label{sec:cond}
\vspace{-0.25cm}

%\ming{It seems why EB-C is a word level quantification is not explicitly explained? EB-bleu is a sequence level is quite evident, but still can have a systematic explanation on the naming. } \ming{see also the comments in sec 6.3}


%This problem also causes EB-bleu to be inapplicable for seq2seq tasks (more detail in Appendix \ref{app:ebbleu_not_seq2seq}). 
%(2) Since the computation of EB-bleu involves the generation of a partial sentence $W_{l+1:L}$, one could argue that exposure bias also takes effect during this partial generation both when $P_M$ or $P_D$ is used as $P_H$, leading to little difference in the sequence-level quality of generation. 


\vspace{-0.25cm}
\subsection{Approach}
\label{sec:ebc_defintion}
\vspace{-0.25cm}

%We design a quantification method to measure the model's \textbf{conditional} generation quality. 
Again, let $P_H \in \{P_M, P_D\}$ denote the prefix distribution. With a given prefix length $l$, we first define the \textit{conditional generation deviation} (CGD) as the expected distance, measured by metric $d$, between $P_M$ and $P_D$ conditioned on the prefix samples from $P_H$: 
%the conditional generation deviation (CGD) with prefix distribution $P_H$ for $P_M$ using metric $d$ as:
\begin{align}
\label{eq:cgd}
\begin{split}
    \text{CGD}({M|H}, l, d) = \mathop{\mathbb{E}}_{W_{1:l} \sim P_{H}}[d(P_{M}(\cdot\ |\ W_{1:l}), P_{D}(\cdot \ |\ W_{1:l}))]
%    \text{CGD}({M|H}, l, d) = \mathop{\mathbb{E}}_{W_{1:l} \sim P_{H}}[d(P_{M}^{W_{l+1}  | W_{1:l}}, P_{D}^{W_{l+1} | W_{1:l}})]
\end{split}
\end{align}
A smaller CGD value suggests a higher-quality conditional word distribution. 
%CGD equals $0$ if $P_M$ equals $P_D$ as defined by the distribution metric $d$.
%where we assume that we have access to $P_{D}(\cdot \ |\ W_{1:l})$, and use it to measure the quality of the model's conditional distribution for $W_{l+1}$. 
For the choice of the distance metric $d$, in addition to the standard $d_\text{TV}$ and $d_\text{JS}$ metrics, we introduce the \textit{greedy decoding divergence} ($d_\text{GD}$) defined as: 
\begin{equation}
\label{eq:dgd}
    d_\text{GD}(P,Q) = \mathbbm{1}(\argmax_iP_i \neq \argmax_iQ_i)
\end{equation}
\vspace{-0.25cm}

where $\mathbbm{1}$ is the indicator function, $P,Q \in \mathcal{P}$, $d_\text{GD}$\footnote{$d_\text{GD}$ qualifies as a pseudo-metric in mathematics.} reflects the model's accuracy with greedy decoding. 

%\ming{to me, the key difference between the two proposed metric is more like conditional and marginal. it is not clear not me why it is named sequence-level and word-level. and I'm wondering why not abstract the distance metric in the EB-bleu like this one.}

Similar to the case of EB-bleu, exposure bias should induce a significant gap between $\text{CGD}({M|M}, l, d)$ and $\text{CGD}({M|D}, l, d)$. We now define a new word-level quantification metric for exposure bias at prefix length $l$ with metric $d$ to be:
\begin{equation}
\label{eq:eb-c-main}
    \text{EB-C}(M, l, d)=\tfrac{\text{CGD}(M|M, l, d)}{\text{CGD}({M|D}, l, d)}
\end{equation}
EB-C describes the relative gain in CGD value when the prefix distribution is replaced by $P_D$ from $P_M$. The measurements of EB-C can be interpreted in a similar way to EB-bleu: 
A large value of EB-C would indicate a serious impact of exposure bias; While a value close to 1 would suggest that exposure bias only has a minor effect.

%For our definition of EB-C, a natural question is why we only focus on the generation distribution of the very next word. The reason is we want to precisely measure how the error caused by the history part affect the generation part, by keeping them separate. If we measure the deviation of, for example, two sampled tokens, the definition will be confusing: Because the second sampled token will be affected not only by the accumulated error induced by the history (sampled from the model), but also by the first generated token as history. To get a better understanding of the intuition behind the definition of EB-C, we  recommend readers to read Appendix \ref{sec:appmoresampleinspection} about our NMT experiment.

Since the computation of CGD (Equation \ref{eq:cgd}) requires access to the data distribution $P_D$, in the next section we first consider experiments in a synthetic setting, where a existing model is used as $P_D$.

\vspace{-0.25cm}
\subsection{Synthetic Experiments and Discussion}
\label{sec:ebc_synthetic}
\vspace{-0.25cm}

In text-GAN literature \citep{yu2016seqgan,rankgan17}, a randomly-initialized one-layer LSTM model with a hidden dimension of 32 is usually used as $P_D$ in synthetic experiments (we denote this setting as $M^\text{rand}_{32}$). However, the model is small-scale and does not reflect any structure existing in real-world text. To improve upon this approach, we train a standard MLE model on the EMNLP-news data, and use it as $P_D$ for our synthetic setting. The model is a one-layer LSTM LM with a hidden dimension of 512. 

%We denote the data model ($P_D$) as $M^\text{news}_\text{512}$.

%(described in Appendix \ref{app:ebm-exp})
 We then train two LSTM LM ($P_M$) with different capacities using samples from the data model, with the standard MLE objective\footnote{The reproducing code is provided in supplementary materials.}. One is a one-layer LSTM with a hidden dimension of 512 (denoted as LSTM-512), the other one has a hidden dimension of 32 (denoted as LSTM-32). The small model scale of LSTM-32 should make it difficult to fully recover the data model. We show test-set perplexity results of the trained models in Appendix \ref{app:pplofmodels}. It is shown that both the LSTM-32 and LSTM-512 models has worse perplexity than the data model, indicating that the data model is not fully recovered by the training process. Finally, EB-C is calculated using 100k samples from $P_M$ and $P_D$.  
 %\ming{this paragraph need refinements. the definition of $M^\text{news}_\text{512}$ is obtrusive. the logic here is not smooth.} 

%We train $P_M$ for 100 epochs using the Adam optimizer with learning rate 0.001. In each epoch, 250k sentences (same to the size of the original EMNLP-news data) of length $L=50$ are sampled from $P_D$ as training data to avoid over-fitting. 

% \footnote{We show that we can get stable measurements using 100k samples in Appendix \ref{app:auxplots}.}

\begin{table}[]
\centering
\begin{tabular}{c|cccccc}
\hline
prefix length         & 20              & 30              & 40              & 50              & 60              \\
\hline
$\text{CGD}(M|D)$           & 0.102 $\pm$ .001 & 0.104 $\pm$ .001 & 0.108 $\pm$ .001 & 0.109 $\pm$ .001 & 0.109 $\pm$ .001 \\
$\text{CGD}(M|M)$           & 0.104 $\pm$ .001 & 0.107 $\pm$ .001 & 0.109 $\pm$ .001 & 0.110 $\pm$ .001 & 0.111 $\pm$ .001 \\
\textbf{$\text{EB-C}(M)$}          & \textbf{1.019} $\pm$ .011 & \textbf{1.027} $\pm$ .013 & \textbf{1.013} $\pm$ .010 & \textbf{1.013} $\pm$ .012 & \textbf{1.011} $\pm$ .011 \\
\hline
$\text{CGD}(M|D_\text{shuf})$ & 0.159 $\pm$ .001 & 0.173 $\pm$ .001 & 0.180 $\pm$ .001 & 0.183 $\pm$ .001 & 0.184 $\pm$ .001 \\
$\text{EB-C}(M|D_\text{shuf})$          & 1.553 $\pm$ .016 & 1.652 $\pm$ .027 & 1.662 $\pm$ .019 & 1.675 $\pm$ .019 & 1.681 $\pm$ .019 \\
\hline
\end{tabular}
%\captionsetup{justification=justified,singlelinecheck=false}
\caption{EB-C measurements with $d_\text{JS}$ as metric for the transformer synthetic setting. We have also tried longer prefix length (e.g. 80 or 100), and get very similar observations. The observations with metric $d_\text{TV}$ are also very similar, and is deferred to Table \ref{tab:eb_c_dtv} (Appendix \ref{app:auxiliary_res_plots}).}
\label{tab:eb_c_main_djs}
\end{table}



In Figure \ref{fig:ebc_main_differentmetric}, EB-C measurements with different metrics $d$ are shown. We also show the standard deviation as error bars from 5 runs with different random seeds. It is shown that the two models give similar measurements. The EB-C value has a slowly increasing trend as prefix length increases, which is expected as a consequence of exposure bias, i.e., $P_M$ should deviate farther from $P_D$ as prefix length increases. However, the average value of EB-C is only around 1.01 or 1.02, meaning that the gap between $\text{CGD}({M|M}, l, d)$ and $\text{CGD}({M|D}, l, d)$ is not large. Similar to the EB-bleu measurements, this suggests an insignificant impact from exposure bias. 

%Also, note that in most NLG applications (such as machine translation or image captioning), the generated sequence typically has short length (less than 30). In that range of history length, the EB-C measurements show that exposure bias only has minimal influence (less than 2\%). 

%In Appendix \ref{app:auxplots}, we repeat the experiment for a transformer LM \citep{transformerxl19zihang}, and get very similar EB-C measurements. 
%It matches our intuition: exposure bias is a general auto-regressive LM training topic, and is not directly related to the choice of model architecture.
%These measurements imply a striking conclusion : \textit{(Informal) Even if all the bad effects from exposure bias for MLE LM training are removed, the relative performance gain is at most 3\%. If the sequence length is not very long, the gain is less than 1\%.}.

%Also, note that EB-C stops to show visible growth at around history length 30, we think the reason is that LSTM's current prediction is only affected by a limited length of history (TODO: add cite), so exposure bias stops to become more influential after some point. 


To dive deeper into the cause of the gap in CGD, and also to further validate Hypothesis \ref{hypo:comfort}, we experiment with the prefix distribution $P_H$ being a corrupted versions of $P_M$, denoted as $P_{M^\text{corrupt}}$. We specify a corrupt rate $c \in [0,1]$, and for each word in a sample prefix drawn from $P_M$, we substitute it to a ``noise'' word drawn uniformly from the vocabulary with probability $c$. Consequently, larger $c$ will cause the prefix distribution to deviate farther from the ground-truth $P_D$. In Figure \ref{fig:ebc_cond_nonMLE_js}a, we show CGD measurement with the corrupted prefix of different corrupt rates. Comparing to the small gap between $\text{CGD}({M|M})$ and $\text{CGD}({M|D})$, we observe larger gaps between $\text{CGD}({M|M^\text{corrupt}})$ and $\text{CGD}({M|D})$. This again validates our hypothesis that the mismatch between the prefix distribution $P_M$ and $P_D$ could be not large enough to induce a significant performance loss. 
%In other words, $P_M$ has learned a ``good enough'' distribution that is able to keep the prefix in the well-behaving region during sampling.

%With these observations, we conclude that, in the synthetic setting considered, exposure bias does exist, but is much less serious than it is presumed to be.  The LSTM LM is more robust to the distributional mismatch for $P_H$ than exposure bias claims it to be. 

%\ming{new subsection?}

What kind of model has a large EB-C measurement? We provide a typical toy example LM  with a large EB-C value. However, we argue that this model is unlikely to be a product of MLE training. %\ming{$M^\text{corrupt}$ as $D$, EB-C is also large? From Figure 3. 0.33 / 0.26}
\begin{example}
\label{eg:cond}
Suppose $L=2$, and $V=\{A,B\}$, the ground-truth data distribution is uniform on $\{AA,AB,BB,BA\}$. $P_M$ is crafted as follows: $P_M(W_1=A)=0.9,P_M(W_2=A|W_1=A)=0.9,P_M(W_2=A|W_1=B)=0.5$. Note that the model behaves worse when $W_1=A$, which is of high probability during sampling.
\end{example}

For Example \ref{eg:cond}, we can easily get $\text{CGD}({M|D}, 1, d_\text{TV})=0.2$ and $\text{CGD}({M|M}, 1, d_\text{TV})=0.36$, which gives us $\text{EB-C}(M,1,d_\text{TV})=1.8$. However, this crafted model is unlikely to be an outcome of MLE training. The fact that $P_M(\cdot\ |\ W_1=B)$ is better modeled suggests that in the training data, there are more sentences beginning with $W_1=B$ than $W_1=A$. So MLE training should assign more probability to $P_M(W_1=B)$, not the other way around. From this perspective, the claim of exposure bias seems to be conflicting with the MLE principle. 
%\footnote{If we change to $P_M(W_1=A)=0.1$, $\text{EB-C}(P_M,1,d_{TV})$ will be 0.2, meaning that the model has better conditional generation performance during sampling}

\begin{figure}
  \centering
  \subfigure[CGD for LSTM-512]{\includegraphics[width=0.3\linewidth]{figs/cond_method/synthetic_512Learn512_cgp.pdf}}
  %\caption{CGD measurement (defined in Equation~\ref{eq:cgd}) for corrupted $P_M$ (with $d_\text{TV}$) for the LSTM-512 synthetic experiment.}
  %\label{fig:cgp_cond_H512LearnH512_tvd}\vspace{-0.3cm}
  %\subfigure[CoT]{\includegraphics[width=0.47\linewidth]{figs/cond_method/synthetic_512Learn512_nonMLE_js.eps}}
  \subfigure[RankGAN]{\includegraphics[width=0.32\linewidth]{figs/cond_method/synthetic_H32_rankgan_js_ebc.pdf}}
  \subfigure[ScratchGAN]{\includegraphics[width=0.32\linewidth]{figs/cond_method/fig_ebc_scratchgan.pdf}}
  %\includegraphics[width=0.49\linewidth]{figs/cond_method/synthetic_512Learn512_nonMLE_js.eps}
  %\caption{(a): EB-C measurements (with $d_{JS}$) for comparing non-MLE methods in the LSTM-512 synthetic experiment. (b): EB-C measurements for comparing RankGAN and MLE for the $M^{random}_{32}$ synthetic experiment, the metric used is $d_{JS}$. }\vspace{-0.2cm}
  \vspace{-0.2cm}
  \caption{(a): CGD measurement (defined in Equation~\ref{eq:cgd}) for corrupted $P_M$ (with $d_\text{TV}$) for the LSTM-512 synthetic experiment. Larger level of corruption leads to larger performance gap. (b,c): EB-C measurements (with $d_\text{JS}$) for comparing non-MLE methods in the synthetic experiment. The ScratchGAN model behaves better with model prefix than data prefix.}
  \label{fig:ebc_cond_nonMLE_js}\vspace{-0.3cm}
\end{figure}

Finally, we use EB-C to compare MLE and non-MLE training methods. We compare MLE against ScratchGAN \citep{scratchgan} and RankGAN \citep{rankgan17} in the synthetic setting. The results are shown in Figure \ref{fig:ebc_cond_nonMLE_js}b and \ref{fig:ebc_cond_nonMLE_js}c and implementation details are given in Appendix \ref{app:implementation-nonMLE}. Note that the RankGAN experiments are conducted in the $M^\text{rand}_{32}$ setting\footnote{A MLE-trained model is used as the pre-trained model for the RankGAN generator. The MLE model has an oracle NLL of 8.67, and RankGAN's oracle NLL is 8.55.}, as we find it hard to do a fast implementation of RankGAN for the  LSTM-512 setting. We find that RankGAN and ScratchGAN gives lower EB-C measurements than MLE, which is as expected, as these methods avoid teacher forcing. Most EB-C values in the ScratchGAN case are less than 1, which matches our intuition that GAN models should behave better when fed with model prefixes than data prefixes. On the other hand, EB-C in the RankGAN case is still slightly larger than 1. We believe the reason is that RankGAN still rely on MLE pre-training.
%These result also suggest that EB-C correctly reflect the significance of exposure bias.
%For CoT, at short prefix length, EB-C is even less than 1. We believe the reason is that CoT trys to make the model biased to behave better when fed with model samples. 
%However, SS gives worse EB-C measurements comparing to MLE, which we currently do not have a good explanation. We refer readers to \citet{sscritique18ferenc} for a discussion about the SS objective. 

%Also, note that most non-MLE methods still rely on MLE training in some way (e.g. for pre-training). 

To the best of our knowledge, this is the first direct empirical evidence showing that non-MLE training does indeed avoid the exposure bias problem in that the model behaves better with model prefix. It also suggests that EB-C correctly capture how the training-testing discrepancy affects generation. Note that lower EB-C value does not mean the generation performance is better (e.g., the authors of ScratchGan \citep{scratchgan} acknowledge their performance is still inferior to the MLE baseline). We will revisit this discussion in Section \ref{ref:sec_discussion}.

%Finally, we want to note that although non-MLE algorithms avoid teacher forcing, these algorithms (using GAN or RL) are usually less stable and more difficult to tune. Given that our quantified measurements of exposure bias are insignificant, we think it should be questioned whether adopting these techniques to avoid exposure bias is a wise trade-off. 
%With these observations, we conclude that, in the synthetic setting considered, exposure bias does exist, but is much less serious than it is presumed to be.  The LSTM LM is more robust to the distributional mismatch for $P_H$ than exposure bias claims it to be. 


==> sec_legacy_marginal-method.tex <==
\vspace{-0.25cm}
\section{A (Wrong) Quantification using Marginal Distribution}
\label{sec:marginal}
\vspace{-0.25cm}

In this section, we propose an intuitive and seemingly correct quantification approach using marginal distributions. The approach can be applied to real-world text data experiments, but it has some lethal weak point. The discussion will lead us to our final precise definition of exposure bias in Section \ref{sec:cond}.

\subsection{Method}
Assuming a given history length $l$, we consider the marginal distribution of $W_{l+1}$ from the following three random process:
\begin{itemize}
    \item Draw word sequences of length $L$ from the data distribution $P_D$. Denote the marginal distribution of the random variable at position $l+1$ ($W_{l+1}$) as $P_{D|D}^{l+1}$, where
    \begin{align}
        P_{D|D}^{l+1}(w)
        =\mathbb{E}_{W_{1:l} \sim P_D} [P_{D}(w\ |\ W_{1:l})].
    \end{align}
    \item Draw word sequences of length $L$ from the model distribution $P_M$. Denote the marginal distribution of the random variable at position $l+1$ as $P_{M|M}^{l+1}$, where
    \begin{align}
        P_{M|M}^{l+1}(w)
        =\mathbb{E}_{W_{1:l} \sim P_M} [P_{M}(w\ |\ W_{1:l})].
    \end{align}
    \item First draw $W_{1..l}$ from $P_D$, then draw $W_{l+1}$ from $P_M(\cdot |W_{1..l})$. Denote the marginal distribution of the random variable at position $l+1$ as $P_{M|D}^{l+1}$, where
    \begin{align}
        P_{M|D}^{l+1}(w) = \mathbb{E}_{W_{1:l} \sim P_D} [P_{M}(w\ |\ W_{1:l})].
    \end{align}
\end{itemize}

By the definition of exposure bias, $P_{M|M}^{l+1}$  suffers from the training-testing discrepancy, while $P_{M|D}^{l+1}$ should be closer to the true distribution $P_{D|D}^{l+1}$. To measure this discrepancy, define the marginal generation deviation (MGD) at history length $l$ of history distribution $P_H$ with metric $d$ as
\begin{align}\label{eq:mmd}
    \text{MGD}(P_{M|H}, l, d) = d(P_{M|H}^{l+1}, P_{D|D}^{l+1})
\end{align}
where $P_H \in \{P_M, P_D\}$ denotes the history distribution. MGD measures the deviation of the marginal distribution of $W^{l+1}$ from ground-truth data distribution. 

Finally, we define the \textit{rate of exposure bias} (EB-M) at history length $l$ of model $P_M$ as the ratio (discrepancy) between the MGD measurements when two different history distributions are fed:
\begin{align}
\begin{split}
    \text{EB-M}(P_M, l, d)=\tfrac{\text{MGD}(P_{M|M}, l, d)}{\text{MGD}(P_{M|D}, l, d)}
\end{split}
\end{align}

For MLE-trained models, EB-M\footnote{Note that one can also directly measure $d(P^{l+1}_{M|M}, P^{l+1}_{M|D})$, but in that way, we can not tell which distribution is better.} is expected to be larger than 1, and larger EB-M indicates a more serious exposure bias problem for the trained model. For the metric $d$, we consider two popular probability metrics: total variation distance (denoted as $d_{TV}$), and Jensen-Shannon divergence (denoted as $d_{JS}$).

\vspace{-0.15cm}
\subsection{Experiments and Discussion}
\label{sec:marginal-exp}

In this section, we focus on answering the following question: ``Does the EB-M measurement correctly reflect the significance of exposure bias?'' In short, our answer is \textit{not really.} The problem is that the distortion of the marginal $P_{M|M}^{l+1}$ is not only affected by the presumably existing exposure bias problem alone, but also by the mismatch between the history distribution $P_{M}$ from $P_{D}$ for $W_{1:l}$, which grows with the length of the history. Therefore, even if the measured EB-M is significantly larger than one, we can not conclude that exposure bias causes serious deterioration. We provide an example to illustrate this argument:
\begin{example}
\label{eg:maringal_example}
Suppose $L=2$, and $V=\{A, B\}$. $P_D$ and $P_M$ are crafted as follows: $P_D(AA)=P_D(BB)=0.5, P_D(AB)=P_D(BA)=0$; And $P_M(W_1=A)=1, P_M(W_2=A|W_1=A)=1, P_M(W_2=B|W_1=B)=1$. 
\end{example}

In Example \ref{eg:maringal_example}, $\text{MGD}(P_{M|M},1,d_{TV})=0.5$ and 
$\text{MGD}(P_{M|D},1,d_{TV})=0$, which gives $\text{EB-M}(P_M, 1,d_{TV})=\infty$. However, the only problem $P_M$ has is the mismatch between the history distributions ($P_M$ and $P_D$) for $W_1$.

\begin{figure*}[h]
  \centering
\includegraphics[width=0.5\linewidth]{figs/marginal_method/ebrate_news_js.eps}
\caption{EB-M (with metric $d_{JS}$) comparison for MLE and non-MLE training on EMNLP-News data. For each training method, we show corpus-BLEU \citep{yu2016seqgan} measurement using the test-set as reference set in the legend.}
\label{fig:ebrate_compare_news}
\end{figure*}

The next set of experiments also suggest that EB-M does not precisely reflect exposure bias. On the EMNLP-news data-set (specified in Appendix \ref{app:ebm-exp}), we compare EB-M measurements for several non-MLE training methods with the baseline MLE model. We include results for Scheduled Sampling (SS) \citep{ss15bengio}, Cooperative Training (CoT) \citep{cot18sidi}, and Adversarial Ranking (RankGAN) \citep{rankgan17}. We provide implementation details for non-MLE methods in Appendix \ref{app:implementation-nonMLE}. Intuitively, these methods will cause the model to be \textit{biased} to behave well with model samples as history, instead of data samples. Therefore, we expect EB-M measurement for non-MLE trained models to be smaller than MLE trained models. However, Figure \ref{fig:ebrate_compare_news} shows that the measurements for different training frameworks are almost the same. We believe the reason is that the EB-M measurements are only reflecting the trivial mismatch between the history distributions. 

Is it possible that the original definition of exposure bias \citep{ss15bengio,seqtrainrnn16marc} exactly refers to this mismatch between the model and data history distributions? However, note that this mismatch is inevitable for any imperfect model, and non-MLE training algorithms can not solve it. We believe a better, more precise definition is needed to discriminate exposure bias from this trivial mismatch. Motivated by this view, we propose a second approach in the section below.


==> trash.tex <==
\section{Auxiliary Plots}
\label{app:auxplots}
In Figure \ref{fig:cgp_cond_js_samplenumcompare}, we show that we are able to get stable measurements of EB-C with 100k samples for the LSTM-512 synthetic experiment.

\begin{figure}[h]
  \centering
  \includegraphics[width=0.49\linewidth]{figs/cond_method/synthetic_512Learn512_JS_samplenumcompare.eps}
  \caption{EB-C measurements with different number of samples for the LSTM-512 synthetic experiment.}
  \label{fig:cgp_cond_js_samplenumcompare}
\end{figure}

In Figure \ref{fig:ebrate_different_number_wiki103_tvd} and Figure \ref{fig:ebrate_compare_news_tvd} we provide EB-M measurements with metric $d_{TV}$ discussed in Section \ref{sec:marginal-exp}, the results are similar to those using metric $d_{JS}$.

\begin{figure}[h]
  \centering
  \includegraphics[width=0.49\linewidth]{figs/marginal_method/wiki103_ebrate_mle_numcompare_tvd.eps}
  \caption{EB-M measurements (with metric $d_{TV}$) using different number of samples on wiki103 data.}
  \label{fig:ebrate_different_number_wiki103_tvd}
\end{figure}

\begin{figure}[h]
  \centering
  \includegraphics[width=0.49\linewidth]{figs/marginal_method/ebrate_news_tvd.eps}
  \caption{EB-M (with metric $d_{TV}$) comparison for MLE and non-MLE training on EMNLP-News data. For each training method, we show corpus-BLEU measurement using the test-set as reference set in the legend.}
  \label{fig:ebrate_compare_news_tvd}
\end{figure}

In Figure \ref{fig:ebrate_compare_tf}, we provide EB-C measurements of a 3-layer transformer LM \citep{transformerxl19zihang} with 512 hidden dimension, in the synthetic setting.

\begin{figure}[h]
  \centering
  \includegraphics[width=0.49\linewidth]{nips_rebutall/synthetic_tfLearn512_len50_ebc.eps}
  \caption{EB-C measures for the transformer LM.}
  \label{fig:ebrate_compare_tf}
\end{figure}

%In Figure \ref{fig:ebc_synthetic32_rankgan} we compare EB-C measurements for RankGAN with MLE in a synthetic experiment. The data model is the same as the synthetic setting in \citet{yu2016seqgan}, which is a one-layer LSTM LM with hidden width 32. Note that the MLE model is used as the pre-trained model for the RankGAN generator. The MLE model has an oracle NLL of 8.67, and RankGAN's oracle NLL is 8.55.
%\begin{figure}[h]
%  \centering
%  \includegraphics[width=0.49\linewidth]{figs/cond_method/synthetic_H32_rankgan_js_ebc.eps}
%  \caption{EB-C measurements for comparing RankGAN and MLE for the H32 synthetic experiment, the metric used is $d_{JS}$.}
%  \label{fig:ebc_synthetic32_rankgan}
%\end{figure}

\section{Real-data Experiments for EB-M}
\label{app:ebm-exp}
One problem in the implementation of EB-M is to estimate the described marginal distributions of $W_{l+1}$. We adopt a simple sample-and-count method: $P_{D|D}^{l+1}$ is estimated by the distribution (histogram) of $W_{l+1}$  from a number (to be specified below) of sentences sampled from the data distribution. For $P_{M|M}^{l+1}$ and $P_{M|D}^{l+1}$, we first draw a number of history samples $W_{1:l}$ from the corresponding history model (model distribution and data distribution respectively). We then feed sampled history sequences into the trained model and estimate the marginal distribution of the $(l+1)_{th}$ word by averaging the predicted distribution $P_M(\cdot|W_{1:l})$. 

We measure EB-M for MLE-trained LSTM LM on two popular data-sets: EMNLP-news (EMNLP 2017 WMT News Section), and wikitext-103\footnote{The wikitext-103 data is available at  \url{https://blog.einstein.ai/the-wikitext-long-\ term-dependency-language-modeling-dataset/}.}. For EMNLP-news we set $L=20$, and only use data samples whose length is longer than $L$. The resulting training/validation/test set has 268k/10k/10k sentences. The vocabulary is of size 5k. We use the 10k samples in the test set for evaluation of EB-M. Note that the EMNLP-news data-set is widely used in text GAN literatures \cite{yu2016seqgan, cot18sidi}. We train a one-layer LSTM LM \citep{lstmlm-speech} of hidden dimension 512 as the MLE baseline model for EMNLP-news.

For wikitext-103, we set $L=50$, and regard a paragraph in the original data as a long sentence. Further, we use half of the data for LM training, and utilize the other half for EB-M evaluation. The resulting training/validation/test/evaluation set has 300k/1.5k/1.5k/300k sentences. The vocabulary is of size 50k. We train a two-layer LSTM LM of hidden dimension 1024 as the MLE baseline model for wikitext-103.

For MLE baseline model training, the Adam optimizer is used with learning rate 0.001, no Dropout \citep{droput14nitish} is applied. The model is trained for 100 epochs.

We first measure EB-M on the wikitext-103 data-set, which has large amount of evaluation data. The results are shown in Figure \ref{fig:ebrate_different_number_wiki103}. We provide EB-M measurements with metric $d_{TV}$ in Appendix \ref{app:auxplots}, as they are similar to those using metric $d_{JS}$. It is shown that the measurements become stable when using 100k data/model samples. EB-M has an average value of 1.10, indicating a significant gap between the model's MGD when fed with history from $P_D$ or $P_M$. Further, we observe a steady growth of EB-M along the length of history, which is expected as an outcome of exposure bias.  

\begin{figure}[h]
  \centering
  \includegraphics[width=0.49\linewidth]{figs/marginal_method/wiki103_ebrate_mle_numcompare_js.eps}
  \caption{EB-M measurements (with metric $d_{JS}$) using different number of samples on wikitext-103 data.}
  \label{fig:ebrate_different_number_wiki103}
\end{figure}

%\begin{figure*}[h]
%\subfigure[wikitext-103]{\label{fig:ebrate_different_number_wiki103}\includegraphics[width=0.5\linewidth]{figs/marginal_method/wiki103_ebrate_mle_numcompare_js.eps}}
%\subfigure[EMNLP-news]{\label{fig:ebrate_compare_news}\includegraphics[width=0.5\linewidth]{figs/marginal_method/ebrate_news_js.eps}}
%\caption{(a): EB-M measurements (with metric $d_{JS}$) using different number of samples on wikitext-103 data. (b): EB-M (with metric $d_{JS}$) comparison for MLE and non-MLE training on EMNLP-News data. For each training method, we show corpus-BLEU \citep{yu2016seqgan} measurement using the test-set as reference set in the legend.}
%\end{figure*}

However, as discussed in Section \ref{sec:marginal-exp}, these measurements can only show that the LM does have better (marginal) generation quality when fed with data prefixes, but does not provide informative information for the significance of exposure bias.

\subsection{Marginal or Conditional?}
THINK: Just delete this section

Following our discussion (Section \ref{sec:corpusbleu-discuss}), we wish to focus on comparing the quality of $W_{l+1}$ (instead of $W_{l+1..L}$) when the prefix $W_{1..L}$ is from $P_D$ or $P_H$. The question now is should we consider the marginal distribution $P^{M|H}_{W_{l+1}}$, or the conditional distribution distribution $P_M(\cdot|w_{l+1..L})$? We invite readers to consider to following toy example:

\begin{example}
\label{eg:maringal_example}
Suppose $L=2$, and $V=\{A, B\}$. $P_D$ and $P_M$ are crafted as follows: $P_D(AA)=P_D(BB)=0.5, P_D(AB)=P_D(BA)=0$; And $P_M(W_1=A)=1, P_M(W_2=A|W_1=A)=1, P_M(W_2=B|W_1=B)=1$. 
\end{example}

Now we consider the marginal distribution of $W_2$ when $W_1$ is either from $P_D$ or $P_M$.  $d_{TV}(P^{M|M}_{W_2}, P^D_{W_2}) = 0.5$ 

TODO: calculate TVD

In Example \ref{eg:maringal_example}, $\text{MGD}(P_{M|M},1,d_{TV})=0.5$ and 
$\text{MGD}(P_{M|D},1,d_{TV})=0$, which gives $\text{EB-M}(P_M, 1,d_{TV})=\infty$. However, the only problem $P_M$ has is the mismatch between the history distributions ($P_M$ and $P_D$) for $W_1$.

\small
\begin{align}
\begin{split}
& \text{EB-rate}(l, P_{M}, P_{D})= \\
& \frac{\mathop{\mathbb{E}}_{w_{1..l} \sim P_{M}}[d_{TV}(P_{D}(w_{l+1}|w_{1..l}), P_{M}(w_{l+1}|w_{1..l}))]}{\mathop{\mathbb{E}}_{w_{1..l}  \sim P_{D}}[d_{TV}(P_{D}(w_{l+1}|w_{1..l}), P_{M}(w_{l+1}|w_{1..l}))]}
\end{split}
\end{align}
\normalsize

%\small
\begin{align}
\begin{split}
    \text{EB}(P_{M}, P_{D}) = \frac{1}{L - 1} \sum^{l=L-1}_{l=1} \text{EB}(l, P_{M}, P_{D})
\end{split}
\end{align}
%\normalsize
where EB stands for EB-rate.

we first establish a generation process in Algorithm \ref{alg:gen}, in which $w_{l+1}$ is sampled from the model given history sampled from $P_{history}$.

%The key idea here is that instead of the conditional distribution $P(w_{l+1}|w_{1..l})$, we rely on marginal distribution $P(w_{l+1})$, which can be efficiently estimated from data samples.

\begin{algorithm}
   \caption{$G(P_{model}, P_{hisotry}, l)$}
   \label{alg:gen}
\begin{algorithmic}
   \STATE {\bfseries Input:}  Model distribution $P_{model}$, history (prefix) distribution $P_{history}$, history length $l$
    \STATE Sample $w_{1..l}$ from $P_{history}$
    \STATE Sample $w_{l+1}$ from $P_{model}(\cdot|w_{1..l})$
   \RETURN $w_{l+1}$
\end{algorithmic}
\end{algorithm}


<p>Idx: ${idx_data_4} <strong>Source German: </strong> ${source_data_4} </p>
<p> <strong>Partial Translation: </strong>${context_data_4}</p>
<p> <strong>Choices: </strong>${choice_data_4}</p>
 <crowd-input name="nextword_data_4" placeholder="Just type the index (a number in the set {0,1,2,3,4,5}) of your choice..." required></crowd-input>
 <p> </p> 
<p>Idx: ${idx_model_4} <strong>Source German: </strong> ${source_model_4} </p>
<p> <strong>Partial Translation: </strong>${context_model_4}</p>
<p> <strong>Choices: </strong>${choice_model_4}</p>
 <crowd-input name="nextword_model_4" placeholder="Just type the index (a number in the set {0,1,2,3,4,5}) of your choice..." required></crowd-input>
 <p> </p>

